Simulated annealing with hit-and-run for convex optimization: rigorous complexity analysis and practical perspectives for copositive programming

We give a rigorous complexity analysis of the simulated annealing algorithm by Kalai and Vempala [Math of OR 31.2 (2006): 253-266] using the type of temperature update suggested by Abernethy and Hazan [arXiv 1507.02528v2, 2015]. The algorithm only assumes a membership oracle of the feasible set, and we prove that it returns a solution in polynomial time which is near-optimal with high probability. Moreover, we propose a number of modifications to improve the practical performance of this method, and present some numerical results for test problems from copositive programming.

==> auto_gap_completely_positive.tex <==
\texttt{extremal\_rand\_1}  & -2.234042e-01 &-7.667645e-03& 8.766473e+06 & 3.152000e+03\\
\texttt{extremal\_rand\_2}  & -5.582429e-01 &-1.987634e-02& 9.073317e+06 & 3.412000e+03\\
\texttt{extremal\_rand\_3}  & -5.791724e-01 &-3.596345e-02& 9.334264e+06 & 3.835000e+03\\
\texttt{extremal\_rand\_4}  & -4.467412e-01 &-9.980087e-03& 8.830209e+06 & 3.147000e+03\\
\texttt{extremal\_rand\_5}  & -7.195398e-01 &-5.940056e-03& 8.628287e+06 & 2.957000e+03\\
\texttt{extremal\_rand\_6}  & -1.128917e+00 &-4.307761e-02& 9.438518e+06 & 4.024000e+03\\
\texttt{extremal\_rand\_7}  & -1.310179e+00 &-2.415651e-02& 9.179767e+06 & 3.708000e+03\\
\texttt{extremal\_rand\_8}  & -9.575965e-01 &-6.826558e-02& 9.641288e+06 & 4.277000e+03\\
\texttt{extremal\_rand\_9}  & -8.085663e-01 &-4.236829e-02& 9.416909e+06 & 3.981000e+03\\
\texttt{extremal\_rand\_10} & -5.398830e-01 &-2.967333e-02& 9.236507e+06 & 3.743000e+03\\


==> auto_gap_copositive_long.tex <==
\texttt{bt1} & CUTE & 2 & 4 & 2.141583e-05 & 8.183025e-06 & 1.066920e+04 \\ 
\texttt{bt5} & CUTE & 3 & 6 & 1.841673e-02 & 1.784239e-08 & 6.203900e+04 \\ 
\texttt{bt8} & CUTE & 3 & 10 & 3.878126e-05 & 7.530542e-06 & 4.058860e+04 \\ 
\texttt{try-b} & CUTE & 2 & 2 & 1.205793e-04 & 4.375391e-05 & 7.981800e+03 \\ 
\texttt{dispatch} & MINLPLib & 3 & 5 & 1.248270e-01 & 1.876185e-01 & 6.452650e+04 \\ 
\texttt{ex3\_1\_2} & MINLPLib & 7 & 5 & 4.200951e-01 & 3.475462e-10 & 2.015601e+06 \\ 
\texttt{ex5\_2\_4} & MINLPLib & 7 & 7 & 7.649665e+00 & 1.695456e-08 & 1.703256e+06 \\ 
\texttt{himmel11} & MINLPLib & 5 & 9 & 7.612295e-01 & 3.809915e-02 & 8.267193e+05 \\ 
\texttt{st\_e09} & MINLPLib & 2 & 2 & 6.667014e-01 & 9.504623e-06 & 8.475600e+03 \\ 
%\texttt{st\_e28} & MINLPLib & 5 & 9 & 7.488497e-01 & 8.456938e-02 & 6.334639e+05 \\ 


==> auto_gap_copositive_short.tex <==
\texttt{bt1} & CUTE & 2 & 4 & 8.195733e+00 & 1.676825e+01 & 2.727600e+03 \\ 
\texttt{bt5} & CUTE & 3 & 6 & 7.233854e-02 & 1.702659e-01 & 1.781630e+04 \\ 
\texttt{bt8} & CUTE & 3 & 10 & 9.980202e-04 & 1.605103e-03 & 1.158860e+04 \\ 
\texttt{try-b} & CUTE & 2 & 2 & 5.874023e-02 & 1.082449e-01 & 1.758400e+03 \\ 
\texttt{dispatch} & MINLPLib & 3 & 5 & 3.618493e-01 & 3.595676e-01 & 1.811730e+04 \\ 
\texttt{ex3\_1\_2} & MINLPLib & 7 & 5 & 4.200951e-01 & 1.245180e-09 & 5.005193e+05 \\ 
\texttt{ex5\_2\_4} & MINLPLib & 7 & 7 & 7.649665e+00 & 4.968483e-08 & 4.249695e+05 \\ 
\texttt{himmel11} & MINLPLib & 5 & 9 & 7.049578e-01 & 8.910667e-02 & 1.012020e+05 \\ 
\texttt{st\_e09} & MINLPLib & 2 & 2 & 7.879863e-01 & 2.114233e-01 & 1.882500e+03 \\ 
%\texttt{st\_e28} & MINLPLib & 5 & 9 & 6.743127e-01 & 1.389793e-01 & 1.138376e+05 \\ 

